Conceptualizing the Relationship between AI Explanations and User Agency

We grapple with the question: How, for whom and why should explainable artificial intelligence (XAI) aim to support the user goal of agency? In particular, we analyze the relationship between agency and explanations through a user-centric lens through case studies and thought experiments. We find that explanation serves as one of several possible first steps for agency by allowing the user convert forethought to outcome in a more effective manner in future interactions. Also, we observe that XAI systems might better cater to laypersons, particularly "tinkerers", when combining explanations and user control, so they can make meaningful changes.

==> 0-TODO_LIST.tex <==
%TC:ignore
\noindent

Version: \DTMnow{} $\approx$
9661
words \hfill \reportOnFIXME

{\footnotesize
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}
\tableofcontents
%\listoftables
%\listoffigures
}

% \textbf{\LARGE{TODO\_LIST}}
% \begin{enumerate}

% \item There are a few peculiarities about the organization of this.
% First, ensure that the MAIN .tex and the .bib are ON THE TOP LEVEL AND NAMED THE SAME THING. 
% Failure to do so will make submission to arXiv via automatically download/uploading more complicated. 
% The rest of this file is just some example formattings from old files.

% \end{enumerate}


\textbf{\LARGE{TODO-LIST}}
\FIXME{JED: avoid using the word "algorithm" in these kinds of papers.
There is some research on public reaction to this word (CHI last year, Malin Eiband was on it) AND it isn't really technically correct.
From a discussion with my advanced algorithms professor (Glencora Borradaile), I learned that a procedure like MCTS is best characterized as a "heuristic" because it comes with basically no guarantees on solution quality or convergence speed}

\begin{enumerate}


\item \textbf{Papers to read/cite}
\item I did that! Measuring users' experience of agency in their own action= https://dl.acm.org/doi/abs/10.1145/2207676.2208350
\item How the Design of YouTube Influences User Sense of Agency= https://dl.acm.org/doi/abs/10.1145/3411764.3445467
\item Recommendations and user agency: the reachability of collaboratively-filtered information= https://dl.acm.org/doi/abs/10.1145/3351095.3372866

\item Modify Introduction!!

\item citations:
Vaccaro, 
agency papers from what Dunni sent me (possibly more),
Actionability: can be thought of as "what do I do next with this explanation?", but also "what do I do next with this REVIEW or criticism, etc"
The use of this particular term may be peculiar to me, it is not clear how widespread this is in XAI - seen it different papers but it has diff definition

\item For full paper... Maybe create design pattern that fits this relationship

\item Validation: https://www.mtab.com/blog/validating-a-survey-what-it-means-how-to-do-it
\item https://www.methodspace.com/blog/validating-a-questionnaire
\item Upol Ehsan latest paper on sociotechnical gap https://arxiv.org/abs/2302.00799
\item https://www.microsoft.com/en-us/research/publication/overreliance-on-ai-literature-review/

\end{enumerate}

\newpage
\setcounter{page}{1}
%TC:endignore

==> documentBody/MUSINGS-HowRelated.tex <==
\section{How are Agency and Explanation Related?}
\label{sectionHowRelated}

Studies on designing agency in AI systems, for example, interactive machine learning(IML) have primarily focused on users with technical know-how and in its absence, requires additional technical training for end-users for them to understand and use the provided agentic functions~\cite{smithRenner2020control, dudley2018review}.

The answer to this question is neither straightforward nor known, but we will tease this apart as best we can:

When an entity provides explanations, the explanations tend to increase agency by increasing knowledge, which allows the user to convert intent to outcome in a more effective manner in future interactions.

Thus, one might say that ``Explanations are one way to provide the first steps of agency''; but also that ``they are not the only way.''
Among the reasons for this caveat, agency can also be effected through direct control.

However, it is also not clear that the entity providing explanations always acts in good faith, as opposed to manipulating the explanation consumer in some fashion~\cite{Chromik2019DarkPO}.
As a result, the knowledge and/or agency relationships should not be assumed, but might be considered an ideal case.
Additionally, we do not foreclose on the hypothesis that another statement of the relationship between agency and explanation might be better.
As an example, perhaps agency and explanations might share multiple simultaneous relationships.

\FIXME{JED: Add any other perspectives you would like to add here. Also not sure what is going on with the commented out material below, if you want it for another section}

% Explainability is one of the most commonly proposed foundational characteristic for AI systems~\cite{fjeld2020principled}.
% • Throughly identify interaction specific XAI user needs - Liao et al
% • How should this instance change to get a different prediction Q (pg 56 - viao xai tutorial)
% do i have the "power" to do these changes
% agentic interactions as a way to test explanations
% Explanation can lead to unwarranted trust in model - maybe if user could personally explore
% Examples of translation design from XAI algorithms to XAI UX (pg 83 - viao xai tutorial)

% What-if tool (pg. 50)
% "adapting interactions" questioning the ai - pg 6
% gendermag - tinkering people 

% pg 6 questioning ai - doctor wants 
% can't predefine user explainability need - pg 8 questioning ai
% "Explanations of data were also important in cases where the users could directly manipulate the data to either adapt the usage to better utilize the AI or to improve the AI performance." - pg 8 contd


% THOUGHT - modify from OUTPUT

% pg 9 questioning ai - What if- scenarios; they think only data scientists like this
% weave into system scenarios
% "a desire to gauge AI limitations" - can't do this without - questioning AI

% may be a way we explore contrastive feature

% pg 9 questioning ai - "system, suggesting a new mechanism for an AI system to provide social explanations with regard to other users’ outcomes and actions" - THINK ABOUT COLLECTIVE AGENCY - Ehsan in expanding explainability paper also mentions "crew knowledge" and ST that shows that social validation facilittes AI contestability - - "For instance, suggestions about knowing what happened to other people getting recommendations from the AI systems"

% static explanations, khanna and dodge added (outside) human-only interactive component - aar/ai

% Operationalize

% Contrastive Explanations!!!

%  MAy be against illusory agency - see dark patterns paper

% towards relatable XAI perceptual paper - participants preferred counterfactual samples. I think because control was embedded, they had to click and actively listen

 % using input in AI explanations is already positive \cite{lai2023selective}

%  heard. End users want to be in control [28, 53],
% but what about when systems cannot respect user inputs?

% Lastly, some users might be interested in knowing other people’s experience with the system, suggesting a new mechanism for an AI system to provide social explanations with regard to other users’ outcomes and actions. liao questionning

\subsection{To what extent can we design explainable systems without agency?}
\label{sectionResults}



% 


When we provide agency in a system, it may be impossible to do without explanations.
When we provide explanations, people need a way to use that explanation.
Apart from being able to know what is going on, are you able to use that information to change things in the system.
Actionability is the explanation word for this agency concept.

Vaccaro paper had some nice stuff about illusion of control, what does that mean in terms of actionability? Taking an action vs taking a MEANINGFUL action.
Only used in games to increase user satisfaction, as an example: avatar selection.
Choosing a class might affect my journey through the game, but choosing hair style would not.



Causal explanation - Why someone did a thing; An agentic interaction is based on some kind of forethought.
Each system provides a good explanation can also inform the actions they take.
Mechanism is refining forethought for next action.
(possibly a nice figure to draw here where we have a feedback loop of plan, action, outcome, repeat).

Possible relationship between refining forethought and counter-factual explanation perturbation? Actionability and perturbation?


\subsection{FIXME Something about actionability? seems to warrant a full subsection in here}

SE framing is also about this same kind of loop as the refinement of forethought, with actionability informing it
% actionability/controllabitlity
% software engineering approach: failure detection, fault localization, fix application, fix verification

Software engineering describes modalities moving from \emph{``FIXME lawrance quote about failure, fault loc, fix, verify''}~\cite{FIXME}.
An analogous pipeline applies for humans consuming explanations to analyze AI.
From an agency perspective, raising a complaint which receives redress is superior to simply receiving an explanation showing why things went wrong.
However, \emph{``FIXME groce quote fix parameterized by actions available''}~\cite{FIXME}.


But is laboring over a bug report that one knows not if they just threw it off a cliff truly "agentic"?

actionability (here is my output and you cant change it, you have some influence)...
%explainability (opaque box, map states to actions, or map states to metadata), 

 This is echoed by Shneiderman et al. [158], who discussed the need for interfaces that allow users “to better understand underlying computational pro- cesses” and give users “the potential to better control their (the algorithms’) actions” as one of the grand challenges for HCI researchers.
 [158]  Shneiderman, B., Plaisant, C., Cohen, M., Jacobs, S.,
 Elmqvist, N., \& Diakopoulos, N. (2016). Grand chal-
  lenges for HCI researchers.
(5), 24-25.






% Case Study: explanations with varying levels of actionability
% could add several case studies, based on explanations, reviews, general interactions, etc
% Actionability - may vary depending on user type
% Dis-aggregation of results?

Thought experiment: we take a player we clone them twice, one we break arm, the next we break arm+leg, leave other alone. shuffle around, pick out which is slightly broken, etc.

Thought experiment: 1:1 basketball, pick the winner. Identity, traits, etc. these markers rely on our ability to tie the information to some semantics

Thought experiment: family painting, pick which of these two bad parts are the child's work or the parent who is a shitty artist (e.g., me)




% \boldify{**similarities between agency and explanation}
% \boldify{**current agentic systems and how they use explanations} - i sort of already talk about this in What is Explanation section
\boldify{**current designs of explainable systems and their deficiencies and how designing for agency can fit/benefit the system}
\boldify{for the above, consider explainability goal of interactivity, check \cite{arrieta2020explainable}}
\boldify{can agency be metric for explainable AI}

\boldify{A new way to look at explainable systems may be the rate at which the provided explanations (become causal) and correlate with the action takes in the system?}

%%%%%%%%%%%%%% Maybe there wouldn't be over-reliance on AI if people could verify AI Explanations themselves
% https://www.microsoft.com/en-us/research/publication/overreliance-on-ai-literature-review/

==> documentBody/OLD-Agency.tex <==
\section{What is Agency?}
\label{sectionAgency}

% \FIXME{JED: I'll leave this section mostly in your wheelhouse
% }


% \subsection{What is Agency?}

Agency is a phenomenon that explores how people approach the world. There is an innate need in people to want to be in control of the course of their lives and be able to predict the outcomes of situations, no matter the difficulty \cite{bandura1996reflectionspart1}. According to Loehr, ``a sense of agency'' is the feeling of ``generating and controlling actions and their effects'' \cite{loehr2022sense}. This means an agentic person is aware and in control of their doing of a action and the corresponding results. Wegner and Wheatley introduce the feeling of agency as the ``conscious experience of will'' \cite{wegner1999apparent}. Humans feel a sense of agency when we believe that our ``conscious intention caused a voluntary action'' \cite{wegner1999apparent}. Agency is an internal ``human'' feeling that is outwardly expressed by intentional actions.

A major component of human agency is ``perceived self-efficacy'' \cite{bandura1982self}. According to Bandura \cite{bandura1982self}, perceived self- efficacy of an individual refers to the degree of belief an individual has in the skills they possess to achieve or complete a task in a specified environment, in a defined order. 
 % Perceived self-efficacy can be improved upon when people acquire [relevant] new skills to overcome tasks they expected to be difficult \cite{bandura1982self}. 
People decide on their level of perceived self-efficacy through four assessments: 1) successful task completion, 2) observation of other people, 3) verbal persuasion and 4) social influences with successful task completion providing the strongest effect \cite{bandura1982self}. 

If people do not think they have enough control, they would abandon the environment and they would not trust their actions especially in hard situations \cite{bandura1982self}. To keep people engaged, there needs to be ``high perceived self-efficacy in a highly responsive environment'' \cite{bandura1982self}. People need to feel like they can control the outcomes of any event in such an environment. Everyone has agency but some people are more agentic than others due to an ``innate need to control'' \cite{goller2017human}. These people are more likely to look for more information, clarification as well as new experiences in a work environment \cite{goller2017human}.

 
Some additional characteristics that bound and help us critically examine this subjective sense/feeling of agency include priority, consistency and exclusivity \cite{wegner1999apparent}. 
Agency is primarily a relationship between thought and action. After an individual believes they can do a thing, they have to perform an action. In this case, priority means the individual definitely had the intention before the voluntary action occurred, consistency means the action corresponds with the thought or intention and exclusivity means there is no other explanation for the the occurrence of the action.
% %%%%    
% %  this reminds me of explainable ai, explanation is not enough

% Agency can occur on an individual or collective basis. When individuals perform a joint action, they can feel individual and/or collective (joint agency) \cite{loehr2022sense}. The individual perceived self-efficacy of multiple members of a group forms collective efficacy which can lead to meaningful social change \cite{bandura1982self, bandura1996reflections}. 

% % There are different typesOf this joint agency, 
% People can derive individual agency while performing tasks with a partner but in cases where the partner makes the dominant decision, the partner feels a greater sense of agency\cite{loehr2022sense}. Joint agency is fluid and not necessarily, a sum of each individual's agency, people assess joint agency collectively and the sense of joint agency is influenced by coordination between the people in the group\cite{loehr2022sense}. 
% Fribourg et. al \cite{fribourg2020virtual} during a research study, where participants shared and controlled the same virtual avatar, were able to show that the agency a person feels is sensitive to visuo-motor coupling (i.e. the visual outcome matched their own movement) even when there is no agency afforded when performing a joint action\cite{fribourg2020virtual}. 

\subsection*{Designing Agency in Technology}

User agency involves the characteristic that the end-user is in charge of and so, can modify their overall experience with a piece of technology \cite{thue2010player}. 
Control and agency are important
parts of an experience \cite{wright2008aesthetics} with technology, and they play a role in the way people use technology \cite{boudreau2005enacting}.
A technology that affords agency is ``flexible'' to the user's interactions inputs and interests \cite{wyeth2007agency}. 
The control a person has in a typical environment (such as while utilizing technology) can be weighted by 1)the presence of relevant actions 2) the relationship between the actions of a user and the outcome in the environment 3) the ability of a user to predict the outcome of their actions and 4) the ability of the user to trace the cause of an outcome \cite{thompson1998illusions}.

Early 2000s research work in user agency \cite{huh2010incorporating, gillies2004integrating, girgensohn2001home} investigated whether the cubersomeness or complexity of a task affects the need for user agency. They showed that even in events where user agency affected efficiency negatively, users still preferred having control. People found the automated results reasonable but there were still questions about how the system generated its results and how to override them. There is a need for ``balance'' between automation and control \cite{girgensohn2001home}. Gillies and Ballin \cite{gillies2004integrating} introduce the concept of levels of control where these levels are based on the difficulty of the skills required to modify user avatar behaviour. These skills vary from needing to learn programming languages to using already created tools and then subtle controls implicit in other tasks. The cognitive load increases across these levels of control and exposing the highest levels to the user, is detrimental to the convenience people expect from using automated technology.
% 




\subsubsection*{IIusory Agency}

% talk about illusory control too. Some sources: 
% \cite{vaccaro2018illusion}

A technological arena where user agency is paramount is video games. There is contention about how much changes a player should be able to make to the story narrative and finite number of action sequences created by the game designer. 
The best story narratives provide game players the highest level of agency without affecting the narrative's design \cite{day2017agency} but there is a limit to the amount of meaningful changes that be accommodated. 
To circumvent this limit while still creating the best interactive game experience, game designers have started to complement the meaningful agency provided \cite{thue2010player}. 
Day and Zhu \cite{day2017agency} refer to this different method of interaction design as an ``Agency Informing Technique'' (AIT). 
The type of perceived agency experienced by the user due to AITs is called \textit{illusory agency} \cite{maccallum2007illusory}.  
The aim is to provide interactions, that display ``commitment to meaning'' \cite{tanenbaum2009commitment}, that increase a player's sense of agency, but don't necessarily have an impactful effect. Game players are able to perform an action, get an outcome they desire, an outcome that is still in line with the game's narrative, with no consequences. 
Some identified AITs in games include: providing interactions that let game players explore the environment, providing visible impacts/feedback of user choices, a screen assuring players that their actions have effects, etc. \cite{day2017agency}.


Agency has been shown to have positive effects such as 1) improved user experience and satisfaction 2) increased trust etc. in different types of technologies~\cite{???}. It is important that people with low or no technical know-how, who form a large portion of AI systems users or stakeholders, also experience these benefits.  


% CHItaly 
% VL/HCCC 2023
 % - https://conf.researchr.org/track/vlhcc-2023/vlhcc-2023-research-papers


 

==> documentBody/OLD-Explanation.tex <==
\section{What is an Explanation?}
\label{sectionExplanation}

% current research
As a result of the observed concerns outlined previously, researchers have developed bodies of knowledge such as Explainable AI (XAI) and Responsible AI.
The aim of the XAI field is to make current opaque AI methods more ``understandable'' to people without compromising their accuracy metric while Responsible AI  furthers the XAI agenda by considering privacy/security, accountability, and fairness~\cite{arrieta2020explainable}.
While some AI algorithms are \emph{inherently} explainable/transparent (e.g., Bayesian models, simple decision trees, Logistic/Linear Regression), researchers have explored possible techniques called post-hoc methods, for making opaque models explainable.
These techniques can work either on a local (i.e., explaining a single prediction), cohort (i.e., explaining a subset of predictions) or global (i.e., explaining all predictions made by the model) scale.
Existing post-hoc methods include rule-based LIME~\cite{ribeiro2016should} and feature extractive Shapley values~\cite{lundberg2017unified}.   

\FIXME{JED: I'll leave this section mostly in your wheelhouse but check on it from time to time.\\\\
I moved the above paragraph from the introduction since it was really background and removed the rest of this with an iffalse/fi combo because it is much too long right now (4 page limit!). Adjust and delete this comment and commands as desired.}

% \iffalse

Explanation is a human phenomenon that strongly relates with peoples' mental models, understanding and knowledge of ``why an outcome happened''~\cite{keil2006explanation}.
An important characteristic of explanations is the social interactive component \cite{keil2006explanation}. There is usually some level of communication (which may be continuous) occurring between the explain-er and explain-ee.
   


% some 
% Analogies
% "causal structure"
 

% Evaluate explanations based on circularity, relevance, coherence
% order in which we receive explantions may influence the explanations we choose as the better/best one
% In trying to gain an explanatory
% understanding of a system, one stops upon reaching a “working understanding.” - \cite{keil2006explanation}
% illusion of explantory depth - rate understanding, give explanation, rerate understanding


Today, AI systems are a major part of our social environment. People interact with these technologies in various capacities and their inclusion in critical areas has made salient the need for explanations for the output generated by these technologies. The output usually can't be assessed or trusted if the targeted users do not understand how the models underlying these technologies work. To help address this issue, the Explainable AI field examines how AI systems can be more understandable from the user and/or AI algorithm perspectives.

% GDPR - rights to explanation
Research areas in explainable AI can be broadly divided into transparency-based and post-hoc  explainability\cite{dovsilovic2018explainable}.
Transparency-based explainable methods deal with inherently explainable AI models. Examples of these models include linear models, decision trees and rule-based models. AI systems can utilize these simpler models directly or combine them with more difficult methods like random forests and Support Vector Machines (SVM) so that explainability and performance is achieved adequately \cite{dovsilovic2018explainable}.
Post-hoc methods aim to modify complex AI models so that they  provide explanations for their predictions~\cite{dovsilovic2018explainable}.
Examples of AI models that are not inherently explainable in regards to complexity include neural networks (NN), ensemble models, and support vector machines (SVM).
These AI models are powerful and also, feature in a lot of critical systems, so there are earnest efforts to make them more explainable while also maintaining their high accuracy.

Based on the ``focus'' of the explanation in a single system, post-hoc XAI techniques can either be local (providing information about a particular decision) or global (providing information about how the whole model works)~\cite{mueller2019explanation, mueller2021principles}.
There are two main approaches employed by post-hoc XAI techniques to generate explanations: opaque box and transparent box.

\subsubsection*{Opaque box explanation techniques} Opaque box explanation techniques treat the whole AI model as opaque and so, operate at the input/output level of various decision instances.
An example of such post-hoc method is Montavon et al.'s~\cite{montavon2017explaining} use of Taylor expansions to discover the input values that produced a prediction.
Earlier research efforts such as LIME~\cite{ribeiro2016should}, SHAP~\cite{lundberg2017unified},  and LORE~\cite{guidotti2019factual} focused on generating local explanations.
LIME~\cite{ribeiro2016should} perturbs the input at a decision and examines how the output changes, sometimes fitting a simpler model to the decision boundary the observer views because of the perturbations.
SHAP~\cite{lundberg2017unified} generates Shapley values using different approximation methods that tell how important all features are at a particular decision.
Exploring counterfactuals are a possible way to create explanations~\cite{keil2006explanation}. This means values, slightly deviated from the scenario being explained, are observed in order to build a pattern. Some modern explainable AI algorithms such as LORE~\cite{guidotti2019factual} utilize this phenomenon.
LORE~\cite{guidotti2019factual} generates a decision tree classifier for input instances in the area around an AI system's particular decision.
From this decision tree, the system records two observations:
a rule that represents the path from the input to the decision output; and a set of rules that represent input changes that would cause a different decision.
Setzu et al.~\cite{setzu2021glocalx} extend LORE to a global context.
They created a ``model-agnostic'' explanation solution called GLocalX that hierarchically merges similar rule-based local explanations to build a global explanation of how the whole system works.
This ``global explainer'' is a transparent and simpler version (and possible replacement) of the opaque model with comparable accuracy.
Another opaque box explanation technique that provides global explanations is BEEF~\cite{grover2019beef}, which solves a combinatorial optimization problem to obtain ``balanced'' explanations.
% Hendricks et al.~\cite{hendricks2016generating} introduced a ``user-centric'' opaque box technique for image classification.
% The proposed AI model is made up of a standard deep classifier and an explanation mechanism that generates the explanation sentences using LSTM and a loss function that favors inclusion of class-specific information.
% The output result is a ``visual explanation'' that contains attributes of the predicted class as well as the image description.

The main advantage of opaque box approaches is that they do not require access to the inner workings of the system---either because it is too complicated or because the user lacks access permissions (e.g., GPT-3~\cite{dale2021gpt} is only accessible through API calls).
The major drawbacks of these approaches are twofold.
First, each AI decision a user inspects requires the explanation system to re-run.
Second, fitting a second (ostensibly simpler) model to the original model's input-output pairs does not \emph{introspect} on the original model.
Thus, while opaque box approaches are useful for understanding the model, they are ill-suited for debugging.

\subsubsection*{Transparent box explanation techniques} Transparent box explanation techniques are interested in the internal structures and operations of the AI model.
An example of this technique that works for image classification is the deconvolutional network (deconvnet) method introduced by Zeiler and Fergus~\cite{zeiler2014visualizing}.
The deconvnet model \emph{``maps the feature activity in intermediate layers to the input pixel space''}~\cite{zeiler2014visualizing}.
When an image input is initially passed to a CNN during training, each layer generates features to pass as an input to the deconvnet model in that layer.
This method outputs a visualization that shows the parts of the input image that are activated for classification.
A different approach for CNNs, that also helps to measure the degree of its ``interpretability'', is to 
(1) collect a list of human-categorized concepts
(2) compute the features activated in each hidden unit for each concept
(3) align concept-activation pairs.
This approach is called network dissection~\cite{bau2017network, bau2020understanding}.
In Deep Q networks, the learned features  ``map'' to different regions~\cite{zahavy2016graying}.
Upon examination of these regions, applicable rules and policies are identified, forming an explanation of the AI model.

Aside from the feature activity in each layer, one could visualize granular level information such as each neuron's ``multiple facets''~\cite{nguyen2016multifaceted}.
Weidele et al.~\cite{weidele2019deepling} modified this type of visualization system with interaction components such that users could explore ``What If?'' scenarios.
The major advantage of transparent box explanations is their ability to assess and debug the model.

% from the user aspect


\subsection*{Evaluating Explanations}

Explanations are evaluated based on ``goodness'' and ``satisfaction'' ~\cite{hoffman2018metrics} in XAI.
In Hoffman et al.'s work, XAI \emph{researchers} are the main actors performing the goodness approach, by comparing an explanation's content/structure/presentation against accepted criteria and established guidelines.
For example, an XAI researcher could consider where their explanation system follows Amershi et al.'s~\cite{amershi2019guidelines} human-AI interaction guidelines and where it does not.
While this is a worthy approach, there is an inherent danger in leaving the definitions of acceptable explanations to AI developers, who already have a degree of comprehension on AI techniques  \cite{miller2017explainable}. 

The ``satisfaction'' metric is obtained when users assess explanations.
Explanation \emph{consumers} see and use various instances of some type(s) of explanations as they complete a task~\cite{mueller2019explanation}.
One example is Dodge et al.'s lab study, in which participants assessed an AI system's effectiveness using instances of several different types of explanations~\cite{dodge2022people}.
Those authors used the results of the participants' assessments to gain insights into each explanation type's strengths and weaknesses.
Another example is Bondi et al.'s investigation into the effects of a given explanation's communication contents and style on the people in human-AI teams when performing an image classification prediction task~\cite{bondi2022role}.



% -------------------------
% OUR AIM: add new element to explanations (meaningful actionability)


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Explanations contain different types of information, which Lim et al.~\cite{lim2009why} formalized into a set of ``intelligibility types.''
% Intelligibility types have proven helpful as XAI researchers design and evaluate their explanations' content.
% For example, they found people preferring ``Why'' information for unexpected behavior, while in other contexts people prioritize ``What'' information such as in strategy games~\cite{lim2009why, penney2018toward} and smart homes~\cite{castelli2017happened}.
% The Why and Why Not intelligibility types have attracted the most attention from XAI researchers, examining explanations targeted at these types in a variety of domains, including pervasive computing~\cite{vermeulen2010pervasivecrystal}, email classification~\cite{kulesza2011oriented}, database queries~\cite{bhowmick2013not,he2014answering}, news feeds~\cite{cotter2017explaining}, and robotics~\cite{hayes2017improving,lomas2012robots,Rosenthal2016robots}.

% Explanations for how an AI model generates output can exist in different formats (e.g., text~\cite{yessenalina2010automatically,liu2019towards, hendricks2021generating}, saliency-maps~\cite{simonyan2013deep, selvaraju2017grad, brahimi2018deep}, graphs~\cite{kulesza2011my, kulesza2015principles}, timelines~\cite{van2004explainable, core2006building}, etc.).

% Human Bias with explanations (Meg tut: pg 31&2)- confirmation bias, anchoring bias, availability bias, unjustified trust/overtrust

% “The property of ‘being an explanation’ is not a property of statements, it is an interaction. What counts as an explanation depends on what the user needs, what knowledge the user already has, and especially the user's goals. - hoffman et al, 2019” (Meg tut: pg 45)

\subsection*{Centering Users in AI Explanations}
% distance from potential victim leads to unethical behaviour -mittelstadtprinciples
Existing explainable AI (XAI) systems that utilize the opaque-box and transparent-box algorithms described above, usually do not fit the researched characteristics for ``everyday'' explanations understandable to the layman (people outside the AI field)~\cite{mittelstadt2019explaining}.
The explanations the XAI systems produce do not translate into helping users make accurate decisions, readily adopt or trust the AI systems.~\cite{alufaisan2021does, liao2020questioning}.
It is important to involve the social elements of explanations expected by actual end users of the system so that it is useful to them. 

Centering people in AI explanations would require that peculiar human factors are taken into consideration. Two explanation concepts that utilize human attributes include analogies and explanatory styles.
Analogies~\cite{keil2006explanation} can be a useful explanation tool especially as a method of providing user-centric explanations. These analogy-based explanations are provided using concepts familiar to the user. Example-based explanations sometimes use analogies~\cite{liao2020questioning}.
% Explanatory types may also vary as a function of the different uses of explanations
Explanatory styles used to present an explanation can differ based on the user's culture (collectivist vs individualistic), purpose for the explanation or user's cognitive abilities ~\cite{keil2006explanation, wang2019designing}.
% Can start from general/core explanation structure that is filled out based on cultural elements

AI explanations that are created based on human characteristics [which directly affect human explanations] (e.g. reasoning and perception methods, preferences) are more relatable and effective for user decision-making \cite{wang2019designing, zhang2022towards, lai2023selective}.
% more relatable, understandable and effective
In their work about connecting existing XAI algorithms to user expectations for explanations, Liao et al.~\cite{liao2020questioning} show that user needs in explanations may vary based on 1) the reason user needs explainability 2) the stage the user is in their use of the AI system as well as 3) the user's persona. They propose a ``question-driven framework'' that encourages an interactive explanation experience~\cite{liao2020questioning}. Extending this interactive experience with an explainable AI system into a socio-organizational context, using Social Transparency, makes it possible to situate explanations in specific humanistic contexts such that the explanation is more understandable and useful to the user \cite{ehsan2021expanding}.

 
% Another type of human-influenced XAI technique based on how people respond to stimuli was introduced by Zhang and Lim~\cite{zhang2022towards}. Evaluation of their XAI  Perceptual Processing Framework~\cite{zhang2022towards} showed that people

% Ehsan et al.~
% "We presented the XAI Perceptual Processing Framework to unify a set of contrastive, saliency, counterfactual and cues explanations towards relatable explainable AI." - Towards relatable XAI perpetual paper| 1. select salient 2) get meaningful cues 3) combine cues to high level concepts



According to Keil~\cite{keil2006explanation}, ``successful'' explanations serve different functions: 
1) help the explain-ee predict future outcomes 
2) aid problem discovery and solving 3) help the explain-er ``justify and rationalize'' their actions and output
Most AI explanations are designed to only perform function 1 i.e. help people make predictions.
% evaluations are usually only predictions too
To enhance an AI explanation's usefulness, user understanding as well as easy adoptabiility, users should be able to engage in meaningful interrogative dialogue with the explanations provided by an AI system~\cite{mittelstadt2019explaining}. A design mindset of user agency and control would allow for interactive components that support probing and exploration in explainable systems. 

% Also, the user should be able to engage in meaningful dialogue with the AI technique \cite{Mittelstadt:2019:EEA:3287560.3287574}.

% \fi

==> documentBody/OLD-Introduction.tex <==
% IGNOREEEE
% IGNOREEEE
% IGNOREEEE 

\section{Introduction
\draftStatus{1.5}}
\label{sectionIntro}

Complex technologies are commonplace in today's society, with examples including reinforcement learning  and deep neural networks.
Due to the existence of large amounts of data and the increasing effectiveness of these technologies, they are making their way into high-stakes scenarios like medicine~\cite{FIXME}, law-enforcement~\cite{Larson2016}, journalism~\cite{FIXME} and automated vehicles~\cite{FIXME}.
Criticisms have plagued the acceptance of the technologies that use these complex algorithms due to the opaque nature of the algorithms and the erasure of user influence (i.e., creating an automated experience).
For example, the high-stakes scenarios mentioned above traditionally require human experts that go through rigorous training, who are then accountable to human stakeholders.
Thus, it is no surprise that such decision makers prefer worse-performing, interpretable models over opaque models~\cite{Veale2018}.

There is also the widely observed problem of AI systems propagating discriminatory practices it learnt from existing data without appropriate checks and balances or adequate oversight~\cite{pmlr-v81-buolamwini18a, RacistAI, Cliskan2022genderbias}.
Beyond experts, lay-people also desire a level of control and understanding of the complex AI (artificial intelligence) systems that affect them~\cite{woodruff2018}.
The EU report~\cite{GDPR} detailing the necessary characteristics for AI systems aligns with the observations above by highlighting the importance of human agency over these systems and the need for these systems to explain and justify their results.
Fostering appropriate trust in existing users, as well as attracting new users may require the system to go beyond accuracy because people want to be aware of the inner mechanisms of the system, as well as available functionalities for influencing the systems' output. 

% what this paper is about
However, making AI systems more \emph{agentic} is not as widely studied as making them \emph{explainable}.
This paper attempts to describe how designing for agency fits into the explainable AI landscape by examining:
\begin{enumerate}[nosep]
    \item the relationship between agency and explanations
    \item case studies of current agentic AI systems and how they use explanations.
\end{enumerate}




==> margin/OLDexample1.tex <==
\begin{margintable}

	\vspace{30pt}

 \noindent 
  \begin{minipage}{\marginparwidth}
    \centering
\begin{tabular}{@{}p{\columnwidth}@{}}
\hline
\RQ{1} What is the range of user attitudes and behaviors surrounding electricity consumption given an age diverse demographic population?\\\\
\RQ{2} How can we effectively capture and convey these attitudes and behaviors?\\
\hline
\end{tabular}
	\caption{Research Questions for this project.}
	\label{researchQuestions}
  \end{minipage}

  \vspace{50pt}

\noindent	
  \begin{minipage}{\marginparwidth}
    \centering
\begin{tabular}{@{}l|l@{\hspace{4pt}}l@{\hspace{4pt}}l@{}}
	\hline
	\textbf{Tag} & \multicolumn{3}{l@{}}{\textbf{Participant age + gender}}\\
	\hline
	\groupTag{ST1}	  & 18-25M & 18-25M \\ 			%S1 Josie, FIGURE:lightswitch
	\groupTag{ST2}   & 18-25F & 18-25M \\ 			%S1 Karl, FIGURE:thermostat
	\groupTag{ST3}   & 18-25F & 18-25M \\ 			%S2 Josie, FIGURE: picture frame
	\groupTag{ST4}   & 18-25F & 18-25M & 18-25M \\ 	%S2 Ron, FIGURE: personZoom
	\hline
	\groupTag{FM1}	  & 36-45F & 18-25M & 11-17F \\ 	%S1 Ron FIGURE: candle
	\groupTag{FM2}  & 46-55F & 11-17F & 5-10F \\ 		%S2 Karl, FIGURE: flowers
	\hline
	\groupTag{OA1}	  & 55+F & 55+M & 55+M \\ 		%S3 Josie FIGURE: granularity
	\groupTag{OA2}  & 55+F & 55+F & 55+M \\ 		%S3 Karl
	\groupTag{OA3}   & 55+F & 55+M & 55+M \\ 		%S3 Ron, FIGURE: appliance comparison
	\hline
	\end{tabular}
	\caption{Demographic information for households. Note that participants are evenly split with respect to gender.  We will use the ``Tag'' given here to refer to our groups while discussing results (ST = student, FM = family, OA = Older Adult).}
	\label{demographicTable}
  \end{minipage}

\end{margintable}

==> margin/OLDexample2.tex <==

\begin{margintable}
  \begin{minipage}{\marginparwidth}
    \centering
    \footnotesize
%\begin{table*}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{@{}p{\columnwidth}@{}}
\hline
\textbf{Skeleton 1} - \skeletonName{Male Retiree} (age 68) \\
\hline
1. $\bullet$ Primarily motivated by saving money\\
2. $\bullet$ Low computing efficacy\\
3. $\square$ Lives alone (per capita usage is high and privacy settings are not needed)\\
4. $\square$ Large amount of time at home\\
5. $\square$ Possesses potentially outdated appliances \\
6. $\vartriangleright$ Thinks his household is energy efficient\\
7. $\vartriangleright$ Little experience with existing energy feedback solutions\\
8. $\vartriangleright$ Habits are entrenched, needs strong reasons to change\\
\\
\hline
\textbf{Skeleton 2} - \skeletonName{Female Parent} (age 37)\\
\hline
1. $\bullet$ Primarily motivated by environmental concerns\\
2. $\bullet$ Medium computing efficacy\\
3. $\square$ Lives with husband, two kids, and a dog\\
4. $\square$ Works outside of the home\\
5. $\square$ Home is new construction, with energy efficient appliances\\
6. $\square$ Wants to shape good habits for her children\\
7. $\vartriangleright$ Likes to compare energy usage with others\\
8. $\vartriangleright$ Willing to make behavior changes to cut carbon emissions\\
\end{tabular}

	\caption{Persona skeletons 1 and 2.  Each is given a gender, occupation, age, primary motivation, and attitude about their own efficacy. The $\square$ is used to denote a piece of household demographic information, while the $\vartriangleright$ is used for information affecting the persona's behavior change disposition.}
	\label{skeletonTable12}
%\end{table*}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \end{minipage}
\end{margintable}

==> margin/OLDexample3.tex <==
\begin{marginfigure}


\noindent
  \begin{minipage}{\marginparwidth}
    \centering
	\includegraphics[width=.85\columnwidth]{assets/candle}
	\caption{A candle generates two scents, roses if the power consumption is low and cinnamon if consumption is high.  These two scents were chosen because neither is bad, but they are noticeably different. Design by \groupTag{FM1}.}
	\label{candle}
  \end{minipage}


\noindent
  \begin{minipage}{\marginparwidth}
    \centering
	\includegraphics[width=\columnwidth]{assets/granularity}
	\caption{On the rightmost column, a \% based goal can be specified.
		After doing so, the goal is shown as a dotted line going across each row.
		The first row is the total consumption, in terms of dollars, while the rest of the rows are appliance specific information.
		The columns track progress toward the daily, weekly, monthly, and yearly goals. Design by \groupTag{OA1}.}
	\label{granularity}
  \end{minipage}


\end{marginfigure}

